How Penalty Leads to Improvement: a Measurement Study of Wireless Backoff

Despite much theoretical work, different modifications of backoff protocols in 802.11 networks lack empirical evidence demonstrating their real-life performance. To fill the gap we have set out to experiment with performance of exponential backoff by varying its backoff factor. Despite the satisfactory results for throughput, we have witnessed poor fairness manifesting in severe capture effect. The design of standard backoff protocol allows already successful nodes to remain successful, giving little chance to those nodes that failed to capture the channel in the beginning. With this at hand, we ask a conceptual question: Can one improve the performance of wireless backoff by introducing a mechanism of self-penalty, when overly successful nodes are penalized with big contention windows? Our real-life measurements using commodity hardware demonstrate that in many settings such mechanism not only allows to achieve better throughput, but also assures nearly perfect fairness. We further corroborate these results with simulations and an analytical model. Finally, we present a backoff factor selection protocol which can be implemented in access points to enable deployment of the penalty backoff protocol to consumer devices.

==> background.tex <==
\section{Background and Research history}

\subsection{IEEE 802.11 modification}
Ethernet~\cite{metcalfe:ethernet}, designed as a link layer protocol to transmit information over a shared, collisions non-free medium, 
dictated the use of a backoff protocol for \textit{Carrier Sense Multiple Access with Collision Detection (CSMA / CD)} scheme. 
As the technology evolved, Ethernet was applied in more sophisticated scenarios. For instance, Ethernet protocol which was 
successful in coaxial cable networks found its application in local area networks (LAN) built with twisted pair cables and 
switches. As such, Ethernet became a de-facto solution for building complex wired networks in which collision avoidance was 
necessary. 

With a rapid growth of wireless communications technology, which exhibits similar properties as any other shared 
medium access environments, the need for a reliable collision avoidance protocol appeared again. The success of Ethernet 
standard in wired networks became an inspiration and a similar scheme, namely \textit{Carrier Sense Multiple Access with Collision 
Avoidance (CSMA/CA)} -- nowadays a part of IEEE 802.11~\cite{ieee80211:standard} standard -- was suggested as a mechanism 
for congestion control in wireless devices. IEEE 802.11 adopted backoff protocol to implement such a mechanism. Although
backoff scheme remained similar to the one in Ethernet, several key changes were made. First was the way how clients actually backoff. 
If $i$ is the number of successive collisions, then clients randomly choose a backoff time from range $[0, T_i = CW_0\cdot 2^i-1]$, 
where $CW_0$ is the initial contention window, which is non-zero even if no collisions happened before. In Ethernet $CW_0=1$, while 
in IEEE 802.11 it was increased to $32$. Though in both cases backoff time can not exceed $1024$. Second, the maximum number of retries, 
and hence potential collisions, before the data frame is discarded was also changed from $16$ in Ethernet to $7$ in IEEE 802.11. 

IEEE 802.11~\cite{ieee80211:standard} standard specifies three coordination functions which deal with collisions:
Distributed Coordination Function (DCF), Point Coordination Function (PCF), and Hybrid Coordination Function (HCF).
In this paper we focus specifically on DCF because it is a fundamental part of collision resolution procedure. 
In short, according to DCF every station in the IEEE 802.11 network has to wait a special period of time in order to avoid 
collisions. In the basic scheme, after every transmission the receiver station has to wait Short Interframe Space (SIFS) before replying
with an acknowledgment packet (ACK) or send/receive specialized control frames. SIFS is the minimal gap between two consequent 
frames required (i) for the receiver to switch from receiving state to sending and (ii) for the sender to separate frames from each 
other. Other stations should wait at least DCF Interframe Space (DIFS) period of time before sending, during which the network remains idle.
If a collision happens (\eg no ACK frame was received) the station chooses uniformly at random the backoff time, which depends on the current 
contention window. Table~\ref{tbl:ifs} shows the values for minimum and maximum contention window sizes along with the other 
parameters specified in IEEE 802.11 standard for frequency-hopping spread spectrum (FHSS), direct-sequence spread spectrum (DSSS) and 
Orthogonal frequency division multiplexing (OFDM) modulation schemes. 

\begin{table}[t]
\begin{center}
\begin{tikzpicture}
\node (table) [inner sep=0pt] {
\begin{tabular}{l|r|r|r}%\hline
& FHSS & DSSS & OFDM \\\hline
\rowcolor{Gray}Slot time              &    50 $\mu$s  &   20 $\mu$s  &   20 or 9 $\mu$s  \\\hline
SIFS time              &    28 $\mu$s  &   10 $\mu$s  &   10 $\mu$s  \\\hline
\rowcolor{Gray}DIFS time              &   128 $\mu$s  &   50 $\mu$s  &   50 or 28 $\mu$s  \\\hline
%Air propagation time   &     1 $\mu$s  &    1 $\mu$s  &    1 $\mu$s  \\\hline
CWmin                  &    16         &   32         &   32 or 16         \\\hline
\rowcolor{Gray}CWmax                  &  1024         & 1024         & 1024         \\%\hline
\end{tabular}
};
\draw [rounded corners=0.8em] (table.north west) rectangle (table.south east);
\end{tikzpicture}
\end{center}
\caption{Time settings and contention window limits for FHSS, DSSS and OFDM versions of the IEEE 802.11 standard.} 
\label{tbl:ifs}
\end{table}

\begin{comment}
In addition to the basic DCF scheme, a RTS/CTS scheme was introduced in the standard. The key idea was to reduce the number of losses of data frames with full payloads 
as well as solve the hidden terminal problem. Thus, whenever a station sends a message 
period of idle time it may be collided with another. If the message is a frame with full payload the whole data will be lost and information
about the collision will be known only after transmission of such a frame. This is very costly for communication, thus, special ``lightweight'' frames
ready-to-send (RTS) and clear-to-send (CTS) were suggested. Whenever a station wants to send some data, it waits the required DIFS period and sends
a RTS frame instead of a full-payload frame. Another station after receiving a RTS frame (addressed to the station) replies with a CTS frame after SIFS period of time. Hence, all 
collisions happen with RTS/CTS frames, and are almost collision-free in between. Additionally, the RTS/CTS scheme helps to deal with {\it the hidden station problem}
-- when two stations not knowing about the existence of each other communicate with one access point (AP). They sense the network is idle, but AP may be in the communication
phase with another station, when a CTS frame comes from AP these stations will know that AP will be busy for some period of time.
\end{comment}

\subsection{Study of the protocol}

Historically, queuing theory was the first way to look at networking problems from mathematical perspective. 
Today it is partly replaced or reconsidered using game-theoretic approach, which we will briefly touch at the end of 
this section.

\begin{comment}
First we are going to take a view on
backoff protocol based on the queueing theory and after that we will take a look on TCP based on the same theory.
\end{comment}

The study of ALOHA protocol~\cite{abramson:aloha} showed that unslotted protocol had the throughput 
$\gamma e^{-2\gamma}$, while the slotted one had $\gamma e^{-\gamma}$, where $\gamma$ 
is the average accumulated arrival rate on input~\cite{roberts:aloha}. It was considered that the maximum number of
active users on the ground may be $324$ for the unslotted (\ie asynchronous) ALOHA protocol. 
As for the slotted model and for the unslotted model with an infinite number of users,
it was shown that the protocol is unstable~\cite{rosenkrantz:instability}. The analysis was based on  
the study of transient Markov chains and martingales. Other different studies were conducted on the
infinite ALOHA model. All of them, however, indicate instability for an infinite number of users.

More interesting was the study of BEB protocol utilized in the Ethernet.
During the more than thirty years old history of Ethernet it was studied a lot
\cite{aldous:ultimate,hastad:analysis,hastad:analysis2,goodman:stability,fayolle:functional, 
rosenkrantz:some, goldberg:analysis,goldberg:contention,tsybakov:survey}, 
and different models were suggested, starting from infinite models, where the number of stations in the
network is infinite\cite{aldous:ultimate,kelly:stochastic,kelly:number,rosenkrantz:some}, 
ending with more specific cases where only two stations are involved~\cite{goodman:onstability}. 

One of the early studies suggested by Kelly~\cite{kelly:stochastic, kelly:number} used a specific 
infinite model with Poisson incoming rate with parameter $\lambda$. The model assumed an infinite number of stations 
in the network and every station sending at most one message. %$N_t$ is a random process which indicates the number of backlogged messages.
In the first work~\cite{kelly:stochastic} it was shown that for schemes that grow slower than exponential backoff, 
the number of "waiting for the channel" messages goes to infinity ($N_t\to \infty$). 
For an exponential backoff there exists a value $v_c$, such that if the input rate
is greater than this value ($\lambda > v_c$), then $N_t\to \infty$. A lower input rate, however, does not guarantee stability in terms of size of the 
backlog ($\mathrm {E}(N_t)$). The second work~\cite{kelly:number} showed the existence of $v_c$ 
value for the general class of random access schemes.
On the other hand, Aldous~\cite{aldous:ultimate} used a different infinite station model with
backoff scheme working as Poisson processes with different parameters. In his work, Aldous
showed that the backoff protocol (and not only backoff protocol, but acknowledgment-based protocols
in general) is unstable for any packet arrival rate $\lambda>0$. 
Additionally, Rosenkrantz similar to the work in~\cite{rosenkrantz:instability} concerning ALOHA protocol, 
proves that under an infinite user model 
the protocol is unstable \cite{rosenkrantz:some}. The analysis shows that the corresponding Markov
chain is transient using martingales.

However, later Hastad et al.~\cite{hastad:analysis} showed using 
a finite model and Bernoulli input process that the polynomial backoff protocol is stable for
any $\lambda$ in terms of positive recurrence (it contradicts the results of Kelly et al.~\cite{kelly:stochastic}).
They measured stability in terms of average waiting time $W_{ave}$ and average number of waiting messages $L_{ave}$, and showed that
stability of any of these values leads to stability of another. In contrast, they showed that BEB 
(or any exponential backoff) is unstable for the overall input rate $\lambda \ge .567 + \frac1{4N-2}$, 
where $N$ is the number of stations (it contradicts Aldous' result~\cite{aldous:ultimate}). Additionally
the work demonstrated that any linear or sublinear backoff protocol is unstable.
Later, the extended version \cite{hastad:analysis2} had more details on the analysis. The actual analysis
was fully based on the method of potential function 
(in some sources referred to as Lyapunov~\cite{goodman:stability}).
The main achievement of Hastad et al. was that in contrast with early works that considered infinite number of stations, 
they used a model which is closest to a real system, and in that model they gained stability conditions in some cases.

Additionally, Goodman et al.~\cite{goodman:onstability, goodman:stability} performed analysis of a
model with finite number of stations, which is also closer to reality. They analyzed  
the $N$ station model, though, a more exact result has been reached for a two-station model. Its simplified
version says that BEB algorithm is stable for $\lambda_1=\lambda_2\le 0.15$. 
The work of Shenker~\cite{shenker:some}, however, argues with the results of Hastad about stability of polynomial
backoff. It states that polynomial backoff is stable for the whole channel capacity $\lambda<1$, but exponential 
and linear are not.

Finally, it is worth to mention a set of papers on traffic analysis of Ethernet protocol \cite{shoch:measured, 
leland:selfsimilar, boggs:measured}. While the first one~\cite{shoch:measured} gives some early practical 
results for the protocol work, which are widely used in theoretical analysis, another paper~\cite{boggs:measured} 
performs traffic analysis with additional knowledge of theoretical assumptions, and also
gives an answer to which assumptions were adequate and which were not applicable. It also demonstrates the great 
impact on performance that {\it capture effect} has. This effect occurs when one station is able to send with higher 
probability than others (so it unfairly captures the channel).The theoretical work of Hastad et al.~\cite{hastad:analysis2}
utilizes the idea of capture effect during the proof of the theorem on potential function. Self-similarity of Ethernet
traffic was also studied in \cite{leland:selfsimilar}.
 
The second inspiration in the study of backoff protocols came up with the adoption of the exponential backoff scheme 
in IEEE 802.11 protocol~\cite{bharghavan:macaw} and the 
work on performance by Bianchi~\cite{bianchi:performance}. The latter was mainly focused on performance of
the protocol instead of the long-term dependencies (such as stability and ergodicity). Using a set 
of assumptions which later were considered reasonable helped to simplify the study. Two of them were
standard assumptions in theoretical works: stations are identical and time divided into timeslots, while two 
were new. The first of them is that the stations are saturated with messages. It means that a station 
always has messages in the queue to send. It is a natural assumption, as if the station has no messages in the sending queue
then it is most probably performing better than the station with messages in the queue. In many cases the saturated 
model shows worse performance than the unsaturated; however, a study without such assumption creates a lot of
cases that should be considered separately. Lastly, there was an assumption on the steady state of the network work,
\ie the collision probability at any moment of time is identical and equal to $p_c$ (it tends to be true with increase
of the number of stations). This is the strongest restriction of the analysis. Recently a study of this assumption 
was conducted in~\cite{kumar:new}, where the restriction was named "fixed-point equation (FPE)".
The work of Bianchi suggested a corresponding Markov chain model and studied the standard BEB protocol 
implemented in IEEE 802.11. An advanced analysis of the same model with a wide range of exponential backoff schemes
was conducted in the work of Kwak et al.~\cite{kwak:performance}. In that work they used 
non-standard backoff factor $r$, as opposed to standard BEB where contention window increased by a factor of 
$2$ ($CW_0\cdot 2^i$). Instead, the new equation that governed the size of contention window was $CW_0\cdot r^i$. 
By applying this modification they found the optimal value for $r$ and suggested
a model for studying the bounded backoff protocol where the number of failed retries before 
discarding was bounded from above. Before that, classical analysis for finite and 
infinite station models assumed the number of failed retries to be infinitely big.
Based on this analysis an extended schema which differs greatly from the backoff protocol  was suggested in~\cite{song:enhancement,song:analysis}. 
It has the form of adaptive backoff protocol, which takes into
account the load in the network at any moment in time. \todo{Added: Finally, in the work~\cite{lukyanenko:performance} the model of Bianchi/Kwak et al. was extended to general backoff scheme. 
It was that the optimal protocol may be found uniquely (based on number of active stations) for the medium, and
after that optimal backoff protocol may be selected among the ones satisfying optimality conditions. This model
will be discussed in more detail in the next Section.} A recent survey and more bibliographical notes can be 
found in~\cite{cho:fundamentals}.

The development of game theory in computer science field also affected the study of backoff protocols. 
The protocols were reconsidered from the game-theoretical point of view, and the analysis indicated 
that equilibrium behavior is selfish in nature, thus calling for a non-standard backoff 
protocols~\cite{konorski:gametheoretic}. The later work suggested an algorithm for fairness called
CRISP (Cooperation via Randomized Inclination to Selfish/Greedy Play), which is logically based on
Prisoner's Dilemma. Another algorithm to deal with unnecessary selfish behavior was suggested by
Altman et al.~\cite{altman:fair}; to ensure that the misbehaving 
station will receive necessary punishment, \ie, protocol functionality in the presence of jammer.

